Lattice point counting via Einstein metrics

We obtain a growth estimate for the number of lattice points inside any Q-Gorenstein cone. Our proof uses the result of Futaki-Ono-Wang on Sasaki-Einstein metric for the toric Sasakian manifold associated to the cone, a Yau's inequality, and the Kawasaki-Riemann-Roch formula for orbifolds.

==> one.tex <==
%!TEX root = Index page.tex
\section{G.I.T. construction from labelled polytopes}
In this section, we give the notations and properties of toric geometry we needed to state and prove the main theorem. We describe briefly how to construct a polarized toric orbifold from the data of labelled polytope, and the relation between lattice points in the polytope and the Riemann-Roch formula. The details are given in appendix. This section can be skipped on first read. \\

\noindent In this paper,  lets denote
\begin{itemize}
\item $N$ be a rank n free abelian group,
\item $M= Hom(N,\mathbb{Z})$,
\item $N_\real=N\otimes_{\mathbb{Z}} \real$,
\item $M_\real= (N_\real)^{\lor}$,
\item $\Sigma$ is a fan inside $N_\real$,
\item $\Sigma(1)$ is the set of $1$ dimensional cone of $\Sigma$,
\item $d=|\Sigma(1)|$
\end{itemize}

\begin{defin}
A labelled polytope is a pair $(P,\beta)$ where $P\subset M_\real$ is a simple rational polytope, and $\beta: \Sigma_{P}(1) \rightarrow \mathbb{Z_{+}}$ is a map. Where $\Sigma_P$ is the inward pointing normal fan associated to $P$. We also denote $m_\rho=\beta(\rho)$ for $\rho \in \Sigma(1)$, $b_\rho=m_\rho \rho$. Here we also write $\rho$ for the primitive vector contained in the cone $\rho$.
\end{defin}

An example of labelled polytope corresponds to weighted projective space is given in the appendix.\\

Given a labelled polytope, a toric complex orbifold can be constructed via G.I.T. construction. Denoted by 
$$\mathcal{X}_{\Sigma_P} =\lbrack \comp^{d}_{s.s} / K_\comp \rbrack$$

There is also a description in terms of local charts which is given in the appendix.\\

\subsection{construction of line bundles}
In this subsection, starting with a simple polytope without labeling, we consider a $\mathbb{Q}$-Cartier divisor $D$ on the variety $X=X_\Sigma$ associated to $\Sigma_P$.

We may write $$D=\sum_\rho \frac{\lambda_\rho}{m_\rho} D_\rho$$, where $\lambda_\rho, m_\rho \in \inte, m_\rho \neq 0$.\\

According to the $m_\rho$, we may define a labeling $\beta(\rho)= m_\rho$ and construct the corresponding $\mathcal{X}=\mathcal{X}_{(\Sigma,\beta)}$ together with a map $\pi : \mathcal{X} \rightarrow X$ corresponds to forgetting the orbifold structure.\\

We can construct a orbi-line bundles $\mathcal{L}$ on $\mathcal{X}$ according to the divisor $D$. If we further assume $N\cdot D$ is globally generated for some $N$, then we have the following properties:\\

\begin{itemize}
\item $\pi_* \mathcal{L}= \mathcal{O}(D)$;\\
\item $H^i(X_\Sigma, \mathcal{O}(D))=0$ for $i>0$;\\
\item $R^i\pi_* (\mathcal{L})=0$ and $R^i\Gamma (\mathcal{L})=0$ for $i>0$;\\

\end{itemize}

This allows us to count the lattice points for the convex polytope defined by $D$ and gives 
\begin{prop}
we denote $M_D$ be the polytope cut out by $D$, then
$$\#(M_D \cap P)=\Gamma(X, \mathcal{O}(D))=\Gamma(\mathcal{X},\mathcal{L})=\chi(\mathcal{X},\mathcal{L})$$
\end{prop}


In the next section, we are going to compute the number $\chi(\mathcal{X},\mathcal{L})$ using an orbifold version of Riemann-Roch formula, called the Kawasaki Riemann-Roch formula\cite{KW79}. The formula given by V. Guillemin \cite{GU97} is suitable for our purpose. 

